Computing maximally-permissive strategies in acyclic timed automata

Timed automata are a convenient mathematical model for modelling and reasoning about real-time systems. While they provide a powerful way of representing timing aspects of such systems, timed automata assume arbitrary precision and zero-delay actions; in particular, a state might be declared reachable in a timed automaton, but impossible to reach in the physical system it models. In this paper, we consider permissive strategies as a way to overcome this problem: such strategies propose intervals of delays instead of single delays, and aim at reaching a target state whichever delay actually takes place. We develop an algorithm for computing the optimal permissiveness (and an associated maximally-permissive strategy) in acyclic timed automata and games.

==> Makefile <==
all:
	for auxfile in $$(ls *.aux); do \
	  if (grep -q "bibstyle" $${auxfile} && \
	      grep -q "citation" $${auxfile}); then \
	    bibtex $${auxfile} || sleep 1; \
	  fi; \
	done; \
	pdflatex main.tex

main.pdf: main.tex
	pdflatex main.tex
	for auxfile in $$(ls *.aux); do \
	  if (grep -q "bibstyle" $${auxfile} && \
	      grep -q "citation" $${auxfile}); then \
	    bibtex $${auxfile} || sleep 1; \
	  fi; \
	done; \
	grep -q "Rerun to get" main.aux && pdflatex main.tex || true
	grep -q "Rerun to get" main.aux && pdflatex main.tex || true

latex-clean: emacs-clean
	for file in $$(ls *.tex) ; \
	  do \
	    base=`basename $${file} .tex` && \
	    (grep -q "\\documentclass" $${file} && \
	    for ext in log aux out bbl blg out vtc idx ilg ind thm nav toc snm tns cb cb2; \
	      do rm -f $${base}.$${ext}; \
	    done) || true; \
	  done; \
	for file in $$(ls *.log) ; do \
	  base=`basename $${file} .log` && \
	  (grep -q "/$${base}.tex" $${file} && \
	    for ext in log aux out bbl blg out vtc idx ilg ind thm nav toc snm tns; \
	      do rm -f $${base}.$${ext}; \
	    done) || true; \
	  done;
	(grep -q "bibunit" *tex && rm -f bu?.aux bu?.blg bu?.bbl) || true


==> lemme_la_sequence_de_function_cv_vers_notre_permissivite.tex <==

  With the same proofs as in \cite{BFM15} (lemma $5$ and $6$), we can prove that $\forall i \geq 0, \forall \varepsilon >0$, there is a winning permissive strategy $\sigma$ such that for all winning configurations $s_0$, $\calP_{ s_0, \loc_f} \left(\sigma \right) \geq \calP_{i} \left(\sigma\right)  + \varepsilon$, and that for any winnning configuration $s$ and any permissive strategy $\sigma '$ that is winning from $s$, $ \calP_{ s , \loc_f } \left(\sigma'  \right) \leq \lim\limits_{ i \rightarrow + \infty} \calP_{i} \left(s \right) $. We will now prove that for any winning configuration $ \left( \loc, v \right) $, such that the longest run from $\left( \loc, v \right)$ to $ \loc_f$ is $i$, $ \left(  \calP_{j} \left( \loc, v \right) \right)_{ j \geq i}$ is stationary. As this sequence is stationary, $ \left( \calP_{j} \left( \loc, v \right) \right)_{ j \geq i }$ will then be equals to the permissiveness of $\left( \loc, v \right)$. First, this property is trivially true for $i=0$, by definition.
  \\To do so, let $i$ be an arbitrary integer and suppose that this property is true for this integer $i$. Let $ \left( \loc, v \right) $ be a configuration such that the longest run from $\left( \loc, v \right)$ to $ \loc_f$ is $i+1$ and $j \geq i+1$. Then, $ \calP_{ j} \left(\loc, v \right) = \sup_{(I,a)\in\moves(\loc,v)}
 \min(|I|, 
 \inf \{\calP_{j-1}(\loc',v')\mid
 \exists d\in I.\ (\loc,v)\trans[d,a](\loc',v')\})$. $\moves(\loc,v)$ and $\left| I \right|$ do not depend on $j$, and that $\left(\inf \{\calP_{j-1}(\loc',v')\mid
 \exists d\in I.\ (\loc,v)\trans[d,a](\loc',v')\})\right)_{ j \geq i }$ is stationary, as $ \loc'$ is at most $i-1$ transition from $\loc_f$, and $ j-1 \geq i-1$. As a result, $ \left( \calP_{j} \left( \loc, v \right)\right)_{ j \geq i+1 }$  is stationary. As a result, our property is true.

   \begin{enumerate}
 \item The equivalence is trivial for $i=0$, by definition.
 Suppose that the equivalence is true for $i \in \bbN$. Let $( \loc, v )$ be a configuration.

 $\Rightarrow $ Suppose that $\calP_{i+1}(\loc,v) = - \infty $ and that there exists a run of length $i+1$ from $(\loc, v)$ to $\loc_f$. Then, there exists a move $(I, a) \in \moves(\loc,v)$ and a delay $d \in I$ such that $(\loc,v) \stackrel{d,a}{\rightarrow} ( \loc', v') $ and that there is a run of length $i$ from $(\loc', v')$ to $\loc_f$. As a result, $(\{d\}, a) \moves ( \loc,v )$ such that $ (\loc,v) \stackrel{d,a}{\rightarrow } (\loc',v')$. By the induction, $\calP_{i+1} (\loc', v') > - \infty $, so $ \calP_{i} ( \loc, v) > - \infty $. Therefore the implication is true.

 $\Leftarrow$ Suppose that there exists no runs of length $i$ from $( \loc, v)$ to $\loc_f$. Then either $\moves(\loc,v) = \varnothing$ (and then $\calP_{i} (\loc,v ) = - \infty)$ \textbf{or} for all moves $(I,a) \in \moves( \loc,v)$ there exists a delay $d \in I$ such that $(\loc,v) \stackrel{d,a} (\loc',v')$ and there are no runs of length $i$ from $(\loc', v' )$ to $\loc_f$. By the induction equivalence, $ \calP_{i} ( \loc', v' ) = - \infty$, then $ \inf\{ \calP_{i} ( \loc', v' ) \mid d \in I, ( \loc,v ) \stackrel{d,a}{\rightarrow} ( \loc', v') \} = - \infty$ for all $(I,a) \in \moves(\loc,v)$.

 As a result $\calP_{i+1} (\loc,v) = - \infty$ and the induction is true.

 
  \item $ \calP_{i} ( \loc ,v ) = - \infty $ if and only if ($i=0$ and $ \loc \neq \loc_f $) or ($ \moves(l,v) = \varnothing $) or ( $ \exists (I, a) \in \moves(\loc,v)$, $\exists d \in I, (\loc,v) \stackrel{d,a}{\rightarrow} (\loc', v'), \calP_{i-1} ( \loc',v' ) = - \infty$).
  Having no runs of length $i$ from $( \loc, v) $ to $ \loc_f $ is equivalent to ($i=0$ and $ \loc \neq \loc_f$) \textbf{or} ($ \moves(l,v) = \varnothing $) \textbf{or} (There exist $(I,a) \in \moves( \loc,v )$, but for \textbf{any} delay $d \in I$ such that $ (\loc,v ) \stackrel{d,a}{\rightarrow} ( \loc' ,v' )$, there are \textbf{no} runs of length $i-1$ from $( \loc', v')$ to $ \loc_f$).
  By a simple induction, the last property implies that $\calP_{i} (\loc,v) = - \infty$. The two first property trivially implies that $\calP_{i} (\loc,v) = - \infty$.
  
  The equivalence is not true, \EC{contre exemple à donner? En gros, si on a un run possible mais que le delai ne correspond pas au meilleur choix de l'opposant, qui arriverait vers une permissivité - infty.}
  \item $ \calP_{i} ( \loc ,v ) = + \infty $ if and only if ($ \loc = \loc_f $) or ( $ \exists (I, a) \in \moves(\loc,v)$ such that $| I | = \infty $ and $\forall d \in I, (\loc,v) \stackrel{d,a}{\rightarrow} (\loc', v'), \calP_{i-1} ( \loc',v' ) = + \infty$).
  Suppose that $ \loc \neq \loc_f$ and that the property is true for $i-1$.  ( $ \exists (I, a) \in \moves(\loc,v)$ such that $| I | = \infty $ and $\forall d \in I, (\loc,v) \stackrel{d,a}{\rightarrow} (\loc', v'), \calP_{i-1} ( \loc',v' ) = + \infty$) if and only if for any $p \in \bbR+$, there exists $(I,a) \in \moves(\loc,v)$ such that $|I| > p $ and $\forall d \in I, (\loc,v) \stackrel{d,a}{\rightarrow} (\loc', v')$ there is a permissive strategy with permissiveness at least $p$ that is winning from $( \loc',v' )$ within $i-1$ steps. It is equivalent that for any $p \in \bbR+$, there exists a permissive strategy with permissiveness at least $p$ that is winning from $( \loc, v)$ within $i$ steps. 
 
  By induction (Case $i=0$ being trivial by definition), our property is true.
 
  \item If $\loc$ is at most $i$ transition from the goal, $\calP_{i} (\loc,v) = \calP ( (\loc,v) , \loc_f)$, then the equivalence is true.
  \\If $ \loc $ is at more than $i$ transitions from the goal, as $ ( \calP_{j} ( \loc,v))_{j}$ is nondecreasing, $\calP (\loc, v) \geq \calP_{i} (\loc , v)$, then the equivalence is true.
 \end{enumerate}

